Decentralized, Communication- and Coordination-free Learning in Structured Matching Markets

We study the problem of online learning in competitive settings in the context of two-sided matching markets. In particular, one side of the market, the agents, must learn about their preferences over the other side, the firms, through repeated interaction while competing with other agents for successful matches. We propose a class of decentralized, communication- and coordination-free algorithms that agents can use to reach to their stable match in structured matching markets. In contrast to prior works, the proposed algorithms make decisions based solely on an agent's own history of play and requires no foreknowledge of the firms' preferences. Our algorithms are constructed by splitting up the statistical problem of learning one's preferences, from noisy observations, from the problem of competing for firms. We show that under realistic structural assumptions on the underlying preferences of the agents and firms, the proposed algorithms incur a regret which grows at most logarithmically in the time horizon. Our results show that, in the case of matching markets, competition need not drastically affect the performance of decentralized, communication and coordination free online learning algorithms.

==> App_TS_proof.tex <==
\subsubsection{Bounds for Algorithm \ref{alg:prunedTSFinal}}
We now present the lemma before which bounds the number of times agents using Algorithm \ref{alg:prunedTSFinal} will get matched to a suboptimal firm:
\begin{lemma}\label{lem: numMatchingAppTS}
For any agent \(a\in\actSet\) using Algorithm \ref{alg:prunedTSFinal} and \(f\in\subArm_a\), we have 
\begin{align*}
    \avg[\numMatches_{a,f}(T)] \leq \bigo\lr{\TSdep(T,\gap)+ \avg\ls{\sum_{t=1}^{T}\one\lr{\collisionEvent_{a,\stableArm_a}(t) }}}
\end{align*}
where \(\gap = \min_{a,f}\gap_{a}(f)\) and \(\TSdep(T,\gap) = \frac{1}{\gap^2} \log\lr{\frac{1}{\gap}}+\frac{ \log(T)}{\gap^2} + \log(T)\)
\end{lemma}
\begin{proof}
Using the definition of total matchings and Lemma \ref{lem: ChooseF} we obtain 
\begin{align*}
\avg[\numMatches_{a,f}(\horizon)] &= \avg\ls{\sum_{t=1}^{\horizon} \one\lr{ \isMatched_a(t) = 1 , \chosenFirm_a(t) = f }}\\
&\leq \underbrace{\avg\ls{\sum_{t=1}^{\horizon} \one\lr{\isMatched_{a}(t)=1,\TSindex_{a,\stableArm_a}(t)\geq \TSindex_{a,f}(t)(t),\actChoose_{a,\stableArm_a}=0,\actChoose_{a,f}=1}}}_{\text{Term A}}\\&\quad\quad+\underbrace{\avg\ls{\sum_{t=1}^{\horizon}\one \lr{\isMatched_{a}(t)=1,\chosenFirm_a(t)=f,\TSindex_{a,f}(t)(t)\geq \TSindex_{a,\stableArm_a}(t)}}}_{\text{Term B}}   
\end{align*}

Let's first analyze Term \(B\). Define \(\filtration_{t-1} = \{\{\chosenFirm_a(\tau),Y_a(\tau), \reward_a(\tau)\}_{\tau=1}^{t-1}\}_{a\in \actSet}\). We first observe that 
\begin{equation}
\begin{aligned}\label{eq: FactorTS}
    &\one\lr{\isMatched_a(t)=1,\actChoose_{a,f}(t)=1,\actQuery_{a,f}(t)=1, \TSindex_{a,\stableArm_a} \leq \TSindex_{a,f}(t)} \\&\quad = \underbrace{\one\lr{\isMatched_a(t)=1,\actChoose_{a,f}(t)=1,\actQuery_{a,f}(t)=1, \TSindex_{a,\stableArm_a} \leq \TSindex_{a,f}(t),\TSindex_{a,f}(t) < \mean_{a,\stableArm_a}-\epsilon}}_{\text{Term C}} \\ 
    &\quad + \underbrace{\one\lr{\isMatched_a(t)=1,\actChoose_{a,f}(t)=1,\actQuery_{a,f}(t)=1, \TSindex_{a,\stableArm_a} \leq \TSindex_{a,f}(t),\TSindex_{a,f}(t) \geq  \mean_{a,\stableArm_a}-\epsilon}}_{\text{Term D}}
\end{aligned}
\end{equation}

We first provide a bound on Term C. Prior to that let's define some notations. Let's define \(\goodProb_{a,f}^{(s)}(\epsilon) = 1-\cdfUpdate_{a,f}^{(s)}(\mean_{a,\stableArm_a} - \epsilon) \). Furthermore,
conditioned on the event that atleast one arm is pulled, for any agent \(a\) let's define \(\mc{P}_a(t)\) to be the set of arms that are pruned before one is chosen to be played at time \(t\). Moreover let \(\actQueryN_{a,f}(t)\) be a random variable such that \(\actQueryN_{a,f}(t)=1\) iff \(f\) is the firm with maximum index value in all of the non-pruned arms at time \(t\). That is,  
\(
\actQueryN_{a,f}(t) = \one\lr{f\in \argmax_{f'\in\firmSet\backslash \{\mc{P}(t)\cup \{\stableArm_a\}\}} \TSindex_{a,f'}(t)}.
\) Using this the following holds:
\begin{align}\label{eq: TS_Eq1}
    \avg[\text{Term C}] &= \avg[\avg[\text{Term C}|\filtration_{t-1}]] \notag \\ 
    &=\avg[\Pr{\isMatched_a(t)=1,\actChoose_{a,f}(t)=1,\actQuery_{a,f}(t)=1, \TSindex_{a,\stableArm_a} \leq \TSindex_{a,f}(t),\TSindex_{a,f}(t) < \mean_{a,\stableArm_a}-\epsilon | \filtration_{t-1}}]\notag \\  &\quad \quad \leq \avg\ls{\Pr{\TSindex_{a,\stableArm_a} < \mean_{a,\stableArm_a}-\epsilon | \filtration_{t-1}} \Pr{\isMatched_a(t)=1,\actQueryN_{a,f}(t)=1,\TSindex_{a,f}(t)<\mean_{a,\stableArm_a}-\epsilon | \filtration_{t-1}}}
\end{align}

Moreover note that 
\begin{align}\label{eq: TS_Eq2}
    &\Pr{\isMatched_a(t)=1,\actQuery_{a,\stableArm_a}(t)=1,\TSindex_{a,f}(t)(t)<\mean_{a,\stableArm_a}-\epsilon|\filtration_{t-1}} \notag \\ & \quad \quad \geq \Pr{\isMatched_a(t)=1,\actQueryN_{a,f}(t)=1, \TSindex_{a,f}(t)(t)<\mean_{a,\stableArm_a}-\epsilon, \TSindex_{a,\stableArm_a}(t) > \mean_{a,\stableArm}-\epsilon|\filtration_{t-1}} \notag \\ 
    &\quad \quad =  \Pr{ \TSindex_{a,\stableArm_a}(t) > \mean_{a,\stableArm_a}(t-1) -\epsilon|\filtration_{t-1}}\Pr{\isMatched_a(t)=1,\actQueryN_{a,f}(t)=1, \TSindex_{a,f}(t)(t)<\mean_{a,\stableArm_a}-\epsilon | \filtration_{t-1}  } 
\end{align}

Using \eqref{eq: TS_Eq2} in \eqref{eq: TS_Eq1} we obtain the following
 \begin{align*}
     &\avg[\text{Term C}] = 
     \avg\ls{\frac{\Pr{\TSindex_{a,\stableArm_a} < \mean_{a,\stableArm_a}-\epsilon | \filtration_{t-1}}}{ \Pr{ \TSindex_{a,\stableArm_a}(t) > \mean_{a,\stableArm_a}(t-1) -\epsilon|\filtration_{t-1}}}\Pr{\isMatched_a(t)=1,\actQuery_{a,\stableArm_a}(t)=1,\TSindex_{a,f}(t)(t)<\mean_{a,\stableArm_a}-\epsilon|\filtration_{t-1}}}
     \\& \quad \quad \quad = \avg\ls{\frac{1-\goodProb_{a,\stableArm_a}^{(\numMatches_{a,\stableArm_a}(t-1))}(\epsilon)}{\goodProb_{a,\stableArm_a}^{(\numMatches_{a,\stableArm_a}(t-1))}(\epsilon)} \Pr{\isMatched_a(t)=1,\actQuery_{a,\stableArm_a}(t)=1,\TSindex_{a,f}(t)(t)<\mean_{a,\stableArm_a}-\epsilon|\filtration_{t-1}}} \\ 
     &\quad \quad \quad\leq \avg\ls{\frac{1-\goodProb_{a,\stableArm_a}^{(\numMatches_{a,\stableArm_a}(t-1))}(\epsilon)}{\goodProb_{a,\stableArm_a}^{(\numMatches_{a,\stableArm_a}(t-1))}(\epsilon)}\Pr{\isMatched_a(t)=1,\actQuery_{a,\stableArm_a}(t)=1|\filtration_{t-1}}}
 \end{align*}
Further evaluating the expectation of Term C we have:
\begin{align*}
    \avg[\text{Term C}] &= \sum_{t=1}^{T}\avg\ls{\frac{1-\goodProb_{a,\stableArm_a}^{(\numMatches_{a,\stableArm_a}(t-1))}(\epsilon)}{\goodProb_{a,\stableArm_a}^{(\numMatches_{a,\stableArm_a}(t-1))}(\epsilon)} \one\lr{\actQuery_{a,\stableArm_a}(t)=1, \actChoose_{a,\stableArm_a}(t)=1, \isMatched_a(t) = 1 }} \\
    &= \sum_{t=1}^{T}\sum_{s=1}^{t} \avg\ls{ \frac{1-\goodProb_{a,\stableArm_a}^{(s)}(\epsilon)}{\goodProb_{a,\stableArm_a}^{(s)}(\epsilon)} \one\lr{\actQuery_{a,\stableArm_a}(t)=1, \actChoose_{a,\stableArm_a}(t)=1, \isMatched_a(t) = 1, \numMatches_{a,\stableArm_a}(t-1) =s }  } \\ 
    &\leq  \avg\ls{\sum_{s=1}^{T}\frac{1-\goodProb_{a,\stableArm_a}^{(s)}(\epsilon)}{\goodProb_{a,\stableArm_a}^{(s)}(\epsilon)} \sum_{t=s+1}^{T} \one\lr{\numMatches_{a,f}(t-1)=s, \numMatches_{a,f}(t)= s+1}} \\ 
     &\leq \sum_{s=0}^{\infty}\frac{1-\goodProb_{a,\stableArm_a}^{(s)}(\epsilon)}{\goodProb_{a,\stableArm_a}^{(s)}(\epsilon)}\\
     &\leq{ \frac{1}{\epsilon^2} \log(\frac{1}{\epsilon})}
\end{align*}
where the last inequality is due to \cite{lattimore2020bandit}\footnote{This inequality is an }.
Now let's look at Term D. Let's set of time indices when \(\mc{J}_{a,f} = \{t: \goodProb_{a,f}^{(\numMatches_{a,f}(t-1))}(\epsilon)> 1/T\}\). 
\begin{align*}
     \avg[\text{Term D}] &=\sum_{t=1}^{T}\avg\ls{\one\lr{\isMatched_a(t)=1,\actChoose_{a,f}(t)=1,\actQuery_{a,f}(t)=1, \TSindex_{a,\stableArm_a} \leq \TSindex_{a,f}(t),\TSindex_{a,f}(t) \geq  \mean_{a,\stableArm_a}-\epsilon}} \\ 
     &\leq \underbrace{\sum_{t\in\mc{J}_{a,f}} \avg\ls{ \one\lr{ \isMatched_a(t) = 1, \actChoose_{a,f}(t)= 1 }}}_{\text{Term E}}  + \underbrace{\sum_{t\not\in \mc{J}_{a,f}} \avg\ls{\one\lr{\TSindex_{a,f}(t) \geq  \mean_{a,\stableArm_a}-\epsilon }}}_{\text{Term F}} 
\end{align*} 
Let's first analyze the Term E above. Note that 
\begin{align*}
    &\sum_{t\in \mc{J}_{a,f}} \one\lr{ \isMatched_a(t) = 1, \actChoose_{a,f}(t)= 1 } \\&\leq  \sum_{t=1}^{T}\sum_{s=1}^{t-1} \one\lr{ \isMatched_a(t) = 1, \actChoose_{a,f}(t)= 1, \goodProb_{a,f}^{s}(\epsilon) > \frac{1}{T}, \numMatches_{a,f}(t-1)=s, \numMatches_{a,f}(t) = s+1} \\ 
    &= \sum_{s=0}^{T-1}\one\lr{\goodProb_{a,f}^{(s)}(\epsilon) > \frac{1}{T}}\sum_{t=s+1}^{T}  \one\lr{\numMatches_{a,f}(t-1)=s, \numMatches_{a,f}(t) = s+1 } \\ 
    &= \sum_{s=0}^{T-1}\one\lr{\goodProb_{a,f}^{(s)}(\epsilon) > \frac{1}{T}} \\ 
    &{\leq \bigo\lr{\frac{ \log(T)}{(\Delta_{a,f}-\epsilon)^2} + \log(T)}}
\end{align*}
where the last property is a property of concentration of normal distribution and is standard in frequentist Thompson sampling analysis. For reader's reference we point to \cite {lattimore2020bandit}.
Next, we bound Term F below: 
\begin{align*}
    \sum_{t\not\in \mc{J}_{a,f}} \avg\ls{\one\lr{\TSindex_{a,f}(t) \geq  \mean_{a,\stableArm_a}-\epsilon }} &= \sum_{t=1}^{T} \avg\ls{\one\lr{\TSindex_{a,f}(t) \geq  \mean_{a,\stableArm_a}-\epsilon, \goodProb_{a,f}^{(\numMatches_{a,f}(t-1))}(\epsilon)\leq \frac{1}{T} }} \\ 
    &=\sum_{t=1}^{T}\avg\ls{\avg\ls{\one\lr{\TSindex_{a,f}(t) \geq  \mean_{a,\stableArm_a}-\epsilon, \goodProb_{a,f}^{(\numMatches_{a,f}(t-1))}(\epsilon)\leq \frac{1}{T} } }|\mc{F}_{t-1}} \\ 
    &= \sum_{t=1}^{T}\avg\ls{\goodProb_{a,f}^{(\numMatches_{a,f}(t-1))}(\epsilon) \one\lr{\goodProb_{a,f}^{(\numMatches_{a,f}(t-1))}(\epsilon)<\frac{1}{T}}} \\ 
    &\leq 1
\end{align*}

Combining the bounds on Term C, Term E and Term F and choosing \(\epsilon = \frac{\gap}{2}\) we have 
\begin{align*}
    \avg[\numMatches_{a,f}(T)] &\leq \bigo\lr{ \frac{1}{\gap^2} \log\lr{\frac{1}{\gap}}+\frac{ \log(T)}{\gap^2} + \log(T) + \avg\ls{\sum_{t=1}^{T} \one\lr{ \actQuery_{a,\stableArm_a}(t)=1, \actChoose_{a,\stableArm_a}(t)=0 } }} \\ 
    &\quad \leq \bigo\lr{ \frac{1}{\gap^2} \log\lr{\frac{1}{\gap}}+\frac{ \log(T)}{\gap^2} + \log(T) + \avg\ls{\sum_{t=1}^{T}\one\lr{\collisionEvent_{a,\stableArm_a}(t) }}}
\end{align*}
where the second inequality is due to Lemma \ref{lem: BoundingTermA}.  This concludes the proof. 
\end{proof}
